The ground calibration of the HERMES-Pathfinder payload flight models

HERMES-Pathfinder is a space-borne mission based on a constellation of six nano-satellites flying in a low-Earth orbit. The 3U CubeSats, to be launched in early 2025, host miniaturized instruments with a hybrid Silicon Drift Detector/scintillator photodetector system, sensitive to both X-rays and gamma-rays. A seventh payload unit is installed onboard SpIRIT, an Australian-Italian nano-satellite developed by a consortium led by the University of Melbourne and launched in December 2023. The project aims at demonstrating the feasibility of Gamma-Ray Burst detection and localization using miniaturized instruments onboard nano-satellites. The HERMES flight model payloads were exposed to multiple well-known radioactive sources for spectroscopic calibration under controlled laboratory conditions. The analysis of the calibration data allows both to determine the detector parameters, necessary to map instrumental units to accurate energy measurements, and to assess the performance of the instruments. We report on these efforts and quantify features such as spectroscopic resolution and energy thresholds, at different temperatures and for all payloads of the constellation. Finally we review the performance of the HERMES payload as a photon counter, and discuss the strengths and the limitations of the architecture.

==> tables/tabletiming.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrr}
\toprule
Mode & GPS lock & Accuracy [ns] & Resolution [ns] \\ \midrule
X-mode & True  & 53.4 & 320 \\
S-mode & True  & 53.4 & 216 \\
X-mode & False & 181 & 320 \\
S-mode & False & 181 & 216 \\
\bottomrule
\end{tabular}
\bigskip
\caption{Timing.} 
\label{tab:timing}
\end{table}
